LRPC codes with multiple syndromes: near ideal-size KEMs without ideals

We introduce a new rank-based key encapsulation mechanism (KEM) with public key and ciphertext sizes around 3.5 Kbytes each, for 128 bits of security, without using ideal structures. Such structures allow to compress objects, but give reductions to specific problems whose security is potentially weaker than for unstructured problems. To the best of our knowledge, our scheme improves in size all the existing unstructured post-quantum lattice or code-based algorithms such as FrodoKEM or Classic McEliece. Our technique, whose efficiency relies on properties of rank metric, is to build upon existing Low Rank Parity Check (LRPC) code-based KEMs and to send multiple syndromes in one ciphertext, allowing to reduce the parameters and still obtain an acceptable decoding failure rate. Our system relies on the hardness of the Rank Support Learning problem, a well-known variant of the Rank Syndrome Decoding problem. The gain on parameters is enough to significantly close the gap between ideal and non-ideal constructions. It enables to choose an error weight close to the rank Gilbert-Varshamov bound, which is a relatively harder zone for algebraic attacks. We also give a version of our KEM that keeps an ideal structure and permits to roughly divide the bandwidth by two compared to previous versions of LRPC KEMs submitted to the NIST with a Decoding Failure Rate (DFR) of $2^{-128}$.

==> applications_to_cryptography.tex <==
\section{Applications to cryptography}\label{sec:applicationsToCrypto}
LRPC codes are good candidates for use in the McEliece cryptosystem
\cite{M78}. As a reminder, the McEliece cryptosystem is a public key
encryption scheme based on coding theory. Basically, the secret key is
the description of a code $\C$ that we can efficiently decode and the
public key is a scrambled description of this code. To encrypt a
message $M$, one computes a codeword $c_M \in \C$ and one adds to it
an error $e$. The ciphertext is $C = c_M+e$. If we know the ``good''
description, we can decode $C$ and recover the message whereas an
attacker has to either apply generic decoding algorithms for arbitrary
codes, which amounts to trying to solve an NP-hard problem, or recover the hidden structure of $\C$.


Ideal LRPC codes are easy to hide since we only need to reveal their
systematic parity-check matrix. Due to their weak algebraic structure,
it is hard to recover the structure of an LRPC code from its systematic form. We can now introduce a new problem on which the security of our cryptosystem is based: 

\begin{problem}[Ideal LRPC codes indistinguishability]\label{prob:IndLRPC} Given a polynomial $P \in \Fq[X]$ of degree $n$ and a vector $\hv \in \Fqm^n$, it is hard to distinguish whether the ideal code $\C$ with the parity-check matrix generated by $\hv$ and $P$ is a random ideal code or whether it is  an ideal LRPC code of weight $d$.

In other words, it is hard to distinguish whether $\hv$ was sampled uniformly at random or as $\xv^{-1}\yv \mod P$ where the vectors $\xv$ and $\yv$ have the same support of small dimension $d$.
\end{problem}

%The ideal LRPC codes are particularly interesting if we choose an irreducible polynomial for $P$. In this case we counter a structural attack against double circulant LRPC which can be found in \cite{HT15}.
In \cite{HT15}, a structural attack against DC-LRPC codes is made by using the divisors of $X^n-1$ in $\Fq[X]$. That is why the ideal LRPC codes are particularly interesting if we choose an irreducible polynomial for $P$. In this case we utterly counter this structural attack.
%We discuss the difficulty of this problem in the subsection \ref{subsubsec:StructuralAttacks}.

In the current state of the art, there is no structural attack against generic LRPC codes : the attack \cite{DT18} on RankSign only works on very specific parameters: it is needed that the weight $d$ of the secret parity-check matrix is less or equal to $\frac{n}{n-k}$, which is not the case for the parameters described in \ref{subsec:Parameters}.

Thus, the most efficient known attack against this problem consists of
searching for a codeword of weight $d$ in the dual $\C^\perp$ of the
LRPC code. Indeed, $\hv = \xv^{-1}\yv \mod P \iff \yv + \xv\hv = 0
\mod P$ so $(\xv|\yv) \in \C^\perp$. The small weight codeword
research algorithms are the same as for the algorithm solving the $\RSD$ problem, so we consider the algorithm of \cite{AGHT17}. However this algorithm is more efficient for LRPC codes than for random codes. Indeed, since an LRPC code admits a parity-check matrix $\Hv$ of small weight $d$, any $\Fq$-linear combinations of the rows of $\Hv$ is a codeword of weight at most $d$ of $\C^\perp$. In the case of Ideal-LRPC codes, the complexity of the algorithm is divided by $q^n$. Thus the complexity of the attack  is $\OO{n^3m^3q^{d\Ceiling{\frac{m}{2}}-m-n}}$.

We can also consider the algebraic attacks using the Groebner bases \cite{LP06}.
The advantage of these attacks is that they are independent of the
size of $q$. They mainly depend on the number of unknowns with respect
to the number of equations. However, in the case $q=2$ the number of
unknowns is generally too high for the algorithms by Groebner basis to
be more efficient than combinatorial attacks described in \ref{best_attacks}. We have chosen our
parameters in such a way so that the best attacks are combinatorial: the expected complexity of the algorithms by Groebner basis is based on the article \cite{BFP09}.


\subsection{An IND-CPA KEM based on the rank metric}
\label{subsec:KEM}


\subsubsection*{Definition of a KEM}
\label{subsubsec:defKEM}
A Key-Encapsulation scheme KEM = $(\KeyGen,\Encap,\Decap)$ is a triple of probabilistic algorithms together with a key space $\mathcal{K}$. The key generation algorithm $\KeyGen$ generates a pair of public and secret keys $(\pk,\sk)$. The encapsulation algorithm $\Encap$ uses the public key $\pk$ to produce an encapsulation $c$, and a key $K \in \mathcal{K}$. Finally $\Decap$ using the secret key $\sk$ and an encapsulation $c$, recovers the key $K \in \mathcal{K}$ or fails and return $\bot$.

We define $\INDCPA$-security of KEM formally via the following experiment, where $\Encap_0$ returns a valid key pair $c^*,K^*$, while $\Encap_1$ return a valid $c^*$ and a random $K^*$.\\[2mm]

\begin{minipage}{0.4\textwidth}
\textit{Indistinguishability under Chosen Plaintext Attack}: This notion states that an adversary should not be able to efficiently guess which key is encapsulated.
\end{minipage}

\fbox{
\begin{minipage}{0.4\textwidth}
$\Exp_{\E,\A}^{\ind-b}(\seck)$
\begin{enumerate}
\item $\param \sets \Setup(1^\seck)$
\item $(\pk,\sk) \sets \KeyGen(\param)$
%\item $(c^*,K_0) \sets \Encap_b(\pk)$
%\item $K_1 \rand \mathcal{K}$
%\item $K^* = K_b$
\item $(c^*,K^*) \sets \Encap_b(\pk)$
\item $b' \sets \A(\GUESS:c^*,K^*)$
\item \comreturn $b'$
\end{enumerate}

\end{minipage}
}

\medskip

\begin{definition}[$\INDCPA$ Security]
	A key encapsulation scheme KEM is $\INDCPA$-secure if for
        every PPT (probabilistic polynomial time) adversary $\advA$,
        we have that
        {\small \[\AdvINDCPA{\KEM}{\advA}:=|\Pr[\INDCPAreal^\advA\Rightarrow 1]-\Pr[\INDCPArand^\advA \Rightarrow 1]|\] is negligible.}
\end{definition}

\subsubsection*{Description of the scheme}
\label{subsubsec:descriptionKEM}
Our scheme contains a hash function $G$ modeled as a Random Oracle Model (ROM).
\begin{itemize}
	\item $\KeyGen(1^\seck)$: 
	\begin{itemize}
		\item choose an irreducible polynomial $P \in \Fq[X]$ of degree $n$.
		\item choose uniformly at random a subspace $F$ of $\Fqm$ of dimension $d$ and sample a couple of 	vectors $(\xv,\yv) \rand F^n \times F^n$ such that $\Supp(\xv)=\Supp(\yv)=F$.
		\item compute $\hv = \xv^{-1}\yv \mod P$.
		\item define $\pk = (\hv, P)$ and $\sk = (\xv,\yv)$.
	\end{itemize}
	\item $\Encap(\pk)$:
	\begin{itemize}
		\item choose uniformly at random a subspace $E$ of $\Fqm$ of dimension $r$ and sample a couple of 	vectors $(\ev_1,\ev_2) \rand E^n \times E^n$ such that $\Supp(\ev_1)=\Supp(\ev_2)=E$.
		\item compute $\cv = \ev_1 + \ev_2\hv \mod P$.
		\item define $K = G(E)$ and return $\cv$.
	\end{itemize}
	\item $\Decap(\sk)$:
	\begin{itemize}
		\item compute $\xv\cv = \xv\ev_1+ \yv\ev_2 \mod P$ and recover $E$ with the RSR algorithm \ref{algo:RSR}.
		\item recover $K = G(E)$.
	\end{itemize}
\end{itemize}


We need to have a common representation of a subspace of dimension $r$ of $\Fqm$. The natural way is to choose the unique matrix $\Mv \in \Fq^{r\times m}$ of size $r\times m$ in its row echelon form such that the rows of $\Mv$ are a basis of $E$.

We deal with the semantic security of the KEM in Section \ref{subsec:secu}.

\begin{figure*}[bt]

\resizebox{\textwidth}{!}{
\fbox{\hspace{-.0cm}%
\begin{minipage}{1.15\textwidth}
\begin{minipage}{.4225\textwidth}
\parbox{\textwidth}{\centering
\underline{Alice}}
\end{minipage} 
\begin{minipage}{.1125\textwidth}
\parbox{\textwidth}{}
\end{minipage} ~
\begin{minipage}{.4225\textwidth}
\parbox{\textwidth}{\centering
\underline{Bob}}
\end{minipage} \\[2mm]
\begin{minipage}{.4225\textwidth}
\parbox{\textwidth}{\centering%
choose $F$ of dimension $d$ at random\\
$(\xv,\yv) \rand F^n\times F^n$, $\hv = \xv^{-1}\yv \mod P$\\[10mm]
$\xv\cv = \xv\ev_1 + \yv\ev_2 \mod P$\\
decode $\sv = \xv\cv$ and recover $E$\\
~\\[2mm]
\fbox{$G\left(\mathbf{E}\right)$}%
}%
\end{minipage} ~
\begin{minipage}{.1125\textwidth}
\parbox{\textwidth}{\centering%
~\\[7mm]
$\xrightarrow{~~~~\mathbf{h}~~~~}$\\[6mm]
$\xleftarrow{~~~~\mathbf{c}~~~~}$\\[8mm]

%$\leftarrow$\textsc{Shared Key}$\rightarrow$
\textsc{Shared Secret}%
}
\end{minipage} ~
\begin{minipage}{.4225\textwidth}
\parbox{\textwidth}{\centering%
~\\[8mm]
choose $E$ of dimension $r$ at random\\
$(\ev_1,\ev_2) \rand E^n\times E^n$ \\
$\cv = \ev_1 + \ev_2\hv \mod P$\\[12mm]
\fbox{$G\left(\mathbf{E}\right)$}%
}
\end{minipage}
\end{minipage}
}%
}
\caption{\label{fig:new_proto}Informal description of our new Key Encapsulation Mechanism. $\mathbf{h}$ constitutes the public key.}
\end{figure*}

\subsection{An IND-CCA-2 PKE based on the rank metric}
\label{subsec:PKE}
%CRS contains a hash function $G$ modeled as a ROM
%
%\begin{itemize}
%	\item KeyGen samples $\vec x, \vec y$ of small weight and outputs a public key $\vec h = \vec x^{-1} \cdot \vec y$.
%	\item To Encrypt a message $M$, one samples $\vec r_1,\vec r_2$ of support $E$ and sends $\vec c=\vec r_1 + \vec h \vec r_2$, and $\vec{d} = M \oplus G(E)$.
%	\item To Decrypt a message, one uses the secret $\vec x, \vec y$ to recovers $E$ from $\vec c$, and $M = \vec d \oplus G(E)$.
%\end{itemize}
Our KEM can be slightly modified to become a PKE cryptosystem.

A Public Key Encryption (PKE) scheme is defined by three algorithms: the key generation algorithm $\keygen$ which takes on input the security parameter $\lambda$ and outputs a pair of public and private keys $(pk,sk)$; the encryption algorithm $\encrypt(pk,M)$ which outputs the ciphertext $C$ corresponding to the message $M$ and the decryption algorithm $\decrypt(sk,C)$ which outputs the plaintext $M$.

Our PKE scheme contains a hash function $G$ modeled as a ROM.
\begin{itemize}
\item $\keygen(1^\lambda)$:
	\begin{itemize}
	\item choose an irreducible polynomial $P \in \Fq[X]$ of degree $n$.
	\item choose uniformly at random a subspace $F$ of $\Fqm$ of dimension $d$ and sample a couple of 	vectors $(\xv,\yv) \rand F^n \times F^n$ such that $\Supp(\xv)=\Supp(\yv)=F$.
	\item compute $\hv = \xv^{-1}\yv \mod P$.
	\item define $pk = (\hv, P)$ and $sk = (\xv,\yv)$.
	\end{itemize}
\item $\encrypt(pk,M)$: 
	\begin{itemize}
	\item choose uniformly at random a subspace $E$ of $\Fqm$ of dimension $r$ and sample a couple of 	vectors $(\ev_1,\ev_2) \rand E^n \times E^n$ such that $\Supp(\ev_1)=\Supp(\ev_2)=E$.
	\item compute $\cv = \ev_1 + \ev_2\hv \mod P$.
	\item output the ciphertext $C = (\cv, M \oplus G(E))$.
	\end{itemize}
\item $\decrypt(sk,C)$:
	\begin{itemize}
	\item compute $\xv\cv = \xv\ev_1+ \yv\ev_2 \mod P$ and recover $E$ with the ideal RSR algorithm \ref{algo:RSR}.
	\item output $M = C \oplus G(E)$.
	\end{itemize}
\end{itemize}

\subsection{Security of our schemes}
\label{subsec:secu}

\begin{theorem}
	Under the \emph{Ideal LRPC indistinguishability} \ref{prob:IndLRPC} and the \emph{Ideal-Rank Support Recovery} \ref{prob:I-RSR} Problems, the KEM presented above in section \ref{subsubsec:descriptionKEM} is indistinguishable against Chosen Plaintext Attack in the Random Oracle Model.
\end{theorem}



\begin{proof}
	We are going to proceed in a sequence of games. The simulator first starts from the real scheme. First we replace the public key matrix by a random element, and then we use the ROM to solve the Ideal-Rank Support Recovery.% It should be noted that the ROM is not used in a programmable way, it is just here 

	We start from the normal game $G_0$:
	We generate the public key $\hv$ honestly, and $E, \cv$ also
	\begin{itemize}
		\item 
	In game $G_1$, we now replace $\hv$ by a random vector, the rest is identical to the previous game. From an adversary point of view, the only difference is the distribution of $\hv$, which is either generated at random, or as a product of low weight vectors. This is exactly the \emph{Ideal LRPC indistinguishability} problem, hence \[\Adv_{\mA}^{G_0} \leq \Adv_{\mA}^{G_1} + \Adv_{\mA}^{\DUPKS}.\]

	\item In game $G_2$, we now proceed as earlier except we receive $\hv, \cv$ from a Support Recovery challenger. After sending $\cv$ to the adversary, we monitor the adversary queries to the Random Oracle, and pick a random one that we forward as our simulator answer to the Ideal-Rank Support Recovery problem. Either the adversary was able to predict the random oracle output, or with probably $1/q_G$, we picked the query associated with the support $E$ (by $q_G$ we denote the number of queries to the random oracle $G$), hence \[\Adv_{\mA}^{G_1} \leq 2^{-\lambda} + 1/q_G \cdot \Adv_{\mA}^{\IRSR}\] which leads to the conclusion.

\end{itemize}
\end{proof}

\begin{theorem}
	Under the \emph{Ideal LRPC indistinguishability} \ref{prob:IndLRPC} and the \emph{Ideal-Rank Support Recovery} \ref{prob:I-RSR} Problems, the encryption scheme presented in section \ref{subsec:PKE} is indistinguishable against Chosen Plaintext Attack in the Random Oracle Model.
\end{theorem}



\begin{proof}
	We are going to proceed in a sequence of games. The simulator first starts from the real scheme. First we replace the public key matrix by a random element, and then we use the ROM to solve the Ideal-Rank Support Recovery.% It should be noted that the ROM is not used in a programmable way, it is just here 

	We start from the normal game $G_0$:
	We generate the public key $\hv$ honestly, and $E, \cv$ also
		\begin{itemize}
			\item 
	In game $G_1$, we now replace $\hv$ by a random vector, the rest is identical to the previous game. From an adversary point of view, the only difference is the distribution of $\hv$, which is either generated at random, or as a product of low weight vectors. This is exactly the \emph{Ideal LRPC indistinguishability} problem, hence $$\Adv_{\mA}^{G_0} \leq \Adv_{\mA}^{G_1} + \Adv_{\mA}^{\DUPKS}.$$

	\item In game $G_2$, we now proceed as earlier except we replace $G(E)$ by random. It can be shown, that by monitoring the call to the ROM, the difference between this game and the previous one can be reduced to the Ideal-Rank Support Recovery problem, so that: \[\Adv_{\mA}^{G_1} \leq 2^{-\lambda} + 1/q_G \cdot \Adv_{\mA}^{\IRSR}.\]

	\item In a final game $G_3$ we replace $C = M \oplus \mathsf{Rand}$ by just $C = \mathsf{Rand}$, which leads to the conclusion.
\end{itemize}
\end{proof}

\subsubsection*{CCA-2 security proof}


When applying the HHK \cite{HHK17} framework for the Fujisaki-Okamoto transformation, one can show that the final transformation is CCA-2 secure such that:
$$\Adv_{\mA}^{\mathrm{CCA-2}} \leq q_G \cdot \delta + q_V \cdot 2^{- \gamma} + \frac{2 q_G + 1}{|\mathcal{M}|} + 3  \Adv_{\mA}^{\mathrm{CPA}}$$
where $q_G$ is the number of queries to the random oracle $G$ and $q_V$ is the number of verification queries.

As our scheme is CPA secure, the last term is negligible, we can handle exponentially large message space for a polynomial number of queries, so the previous is too.

As shown before, our scheme is gamma-spread so again for a polynomial number of verification queries, the term in $q_V$ is negligible.

The tricky term remaining is $q_G \cdot \delta$, this is the product
of the number of queries  to the random oracle, by the probability of
generating an decipherable ciphertext in an honest execution. For real
applications, we want schemes to be correct enough so that the
probability of such an occurrence is very small. This often leads, in
application in running with a probability of a magnitude of
$2^{-64}$. This may seem not low enough for pure cryptographic
security, however it should be noted that this number corresponds to the number of requests adversarially generated where the simulator gives an honest answer to a decryption query, which would mean that a single user would be able to do as many queries as expected by the whole targeted users in a live application, so a little trade-off at this level seems more than fair.

%\subsection{Known Attacks}
%\label{subsec:attacks}
%There are two ways to attack our system: either the opponent can try to recover the structure of the ideal LRPC code by searching a codeword of weight $d$ in the ideal code generated by $\hv$, or he can try to solve an instance of the $\IRSR$ \ref{prob:I-RSR} problem of weight $r$ for a random ideal code.
%
%There exist two types of generic attacks on these problems:
%\begin{itemize}
%\item the combinatorial attacks where the goal is to find the support of the error or of the codeword.
%\item the algebraic attacks where the opponent tries to solve an algebraic system by Groebner basis.
%\end{itemize}
%First, we deal with the combinatorial attacks, both in the generic case and in the ideal LRPC case and in a third subsection we discuss about the algebraic attacks.
%
%\subsubsection*{Generic attacks}
%\label{subsubsec:GenericAttacks}
%In this section, we give the complexity of the best attack on the $\IRSR$ \ref{prob:I-RSR} problem:
%the inputs are a vector $\hv \in \Fqm^n$ which defines the systematic parity-check matrix of an $[2n,n]_{q^m}$ ideal code $\C$, a syndrome $\cv = \ev_1 + \ev_2\hv \mod P$ and an integer $r$ which is the dimension of the support $E$ of $\ev = (\ev_1,\ev_2)$. The goal is to find $E$.
%
%This attack is an improvement of a previous attack described in \cite{GRS16}, a detailed description of the attack can be found in \cite{AGHT17}. For a better understanding, we first describe the first  attack, then the new attack can easily be deduced from it. These attacks do not take account on the ideal structure of the code but in the current state-of-the-art, we do not know any generic combinatorial attack which uses this structure. \\
%
%The first step is to compute a parity check matrix $\Hv$ of size $n \times 2n$ of $\C$ from $\hv$ such that we have the system $\Hv\ev^T= \cv$ of  $n$ equations over $\Fqm$. This step is polynomial so its cost is negligible.\\
%Let $F$ be a subspace of $\Fqm$ of dimension $t$ and $(F_1,\dots, F_t)$ a basis of $F$. We will determine the value of $t$ later. Let us assume that $E \subset F$.
%\[ \Rightarrow \forall i \in [1..2n], e_i = \sum_{j=1}^t \lambda_{ij} F_j \]
%This gives us $2nt$ unknowns over $\Fq$ and we have:
%\begin{IEEEeqnarray}{Cl}
%& \Hv\ev^T = \cv \\
%\Leftrightarrow & \left\lbrace \begin{array}{ccccl}
%H_{1,1}e_1 & + \dots + & H_{1,2n}e_{2n} & = & c_1\\
%\vdots && \vdots &&\vdots \\
%H_{n1}e_1 & +\dots + & H_{n,2n}e_{2n} & = & c_n
%\end{array}\right. \nonumber \\
%\Leftrightarrow & \left\lbrace \begin{array}{ccccl}
%\sum_{j=1}^t \left( \lambda_{1j} H_{1,1} F_j \right. & +\dots +& \left.\lambda_{2n,j}H_{1,2n}F_j \right) & =& c_1 \\
%\vdots && \vdots &&\vdots \\
%\sum_{j=1}^t \left( \lambda_{1j} H_{n-k,1} F_j \right. & +\dots +& \left.\lambda_{2n,j}H_{n,2n}F_j \right) & =& c_n
%\end{array}\right. \label{eqn:RSD_Fqm}
%\end{IEEEeqnarray}
%
%Let $\varphi_i$ the  $i^{th}$ canonical projection from $\Fqm$ on $\Fq$:
%\begin{IEEEeqnarray}{rCCCl}
%\varphi_i & : & \Fqm & \rightarrow & \Fq \nonumber \\
%&& \sum_{i=1}^m x_i \beta_i &\mapsto & x_i \nonumber
%\end{IEEEeqnarray}
%We apply these functions to the $n$ equations of (\ref{eqn:RSD_Fqm}) to obtain
%\begin{IEEEeqnarray}{l}
%\Hv\ev^T = \sv \nonumber \\
%%
%\Leftrightarrow \forall i \in [1..m],\nonumber\\
%  \left\lbrace \begin{array}{ccccl}
%\sum_{j=1}^t \big( \lambda_{1j} \varphi_i(H_{11} F_j)  & +\dots +& \lambda_{nj}\varphi_i(H_{1,2n}F_j) \big) & =& \varphi_i(c_1) \\
%\vdots && \vdots &&\vdots \\
%\sum_{j=1}^t \big( \lambda_{1j} \varphi_i(H_{n,1} F_j) & +\dots +& \lambda_{nj}\varphi_i(H_{n,2n}F_j) \big) & =& \varphi_i(c_n)
%\end{array}\right. \label{eqn:RSD_Fq}
%\end{IEEEeqnarray}
%
%Since we assume $E \subset F$, this system has at least one solution. We want $nm \geqslant 2nt$ to have more equations than unknowns
%$\implies t \leqslant \Floor{\frac{m}{2}}$. To check this assumption, we have to try and solve the system, that's why the complexity of this attack is $\OO{\frac{n^3m^3}{p}}$ where $p$ is the probability that $E \subset F$.\\
%$p$ is equal to the number of subspaces of dimension $r$ in a subspace of dimension $t$ divided by the total number of subspaces of dimension $r$ in $\Fqm$.
%\[ p = \frac{\cg{r}{t}}{\cg{r}{m}} \approx q^{-w(m-t)} \]
%%\commAH{TODO donner le la formule du nb d'ev après la def du support}\\
%By taking $t = \Floor{\frac{m}{2}}$ we obtain a complexity of \[\OO{n^3m^3q^{t\Ceiling{\frac{m}{2}}}}\]
%
%The new attack take account on the $\Fqm$-linearity of the code $\C$. Let $\xv$ be any solution of the system $\Hv\ev^T = \cv$ without consider its weight. Let $\C' = \C + \Fqm\xv$ be the $[2n,n+1]_{q^m}$ code generated by $\C$ and $\xv$. By construction, $\ev \in \C'$ and by $\Fqm$-linearity any multiples $\alpha \ev \in \C', \alpha \in \Fqm$. If $r$ is small, then with overwhelming probability, all the codewords of $\C'$ of weight $r$ are multiple of $\ev$. If we know a codeword $\ev' = \alpha\ev$ of weight $r$ of $\C'$, we can recover $\ev$ then $E$ by solving the equation $\Hv\ev' = \alpha\cv$ of unknown $\alpha \in \Fqm$.
%
%The rest of the algorithm is the same as previously. We choose a subspace $F'$ of dimension $t'$ and assume that $F'$ contains the support $\alpha E$ of a codeword $\alpha \ev$. There are at most $\frac{q^m-1}{q-1}$ subspaces of this form, because $\alpha E = \beta E$ if $\alpha/\beta \in \Fq^*$ and this bound is reached if $m$ is prime, which is always the case in the parameters we have proposed. Since we have $\frac{q^m-1}{q-1}\cg{r}{t'} \ll \cg{r}{m}$, we can approximate the probability $p'$ that $F' \supset \alpha E$ by the product of the probability that $F' \supset E$ by the number of subspaces of the form $\alpha E$
%\[
%p' \approx \frac{q^m-1}{q-1}\frac{\cg{r}{r'}}{\cg{r}{m}} \approx q^{-r(m-t')+m-1}
%\]
%
%Then we express the coordinates of $\alpha \ev$ in a basis of $F'$, which gives us $2nr'$ unknowns over $\Fq$.
%Since $\C'$ is an $[2n,n+1]_{q^m}$ code, the parity-check equations give us $m(n-1)$ equations over $\Fq$, so we need $t' \leqslant \Floor{\frac{m(n-1)}{2n}} = m - \Ceiling{\frac{m(n+1)}{2n}}$ to solve the system. The complexity of the attack is
%\[
%\OO{\frac{(nm)^3}{p'}} = \OO{(nm)^3 q^{r\Ceiling{\frac{m(n+1)}{2n}} - m}}
%\]
%and the gain is almost $q^m$ with respect to the previous attack.
%
%\subsubsection*{Structural attack against ideal LRPC codes}
%\label{subsubsec:StructuralAttacks}
%Let $\C$ be an $[2n,n]_{q^m}$ ideal LRPC code generated by the two polynomials $(\xv,\yv)$ of support $F$ of dimension $d$. Let $\hv = \xv^{-1}\yv$ which generates the systematic parity-check matrix of $\C$. The problem is to recover the structure of $\C$, given only access to $\hv$.
%
%The most efficient known attack is to find a codeword of weight $d$ in the dual code $\C^\perp$ generated by $\hv$. The algorithm described in the previous section is the best known algorithm to solve this problem. However its complexity is better in the case of the dual of an ideal LRPC code than in a random code with the same parameters.
%
%Indeed, let $\Hv$ be the matrix of size $n\time 2n$ generated by $(\xv,\yv)$. By definition, $\Hv$ is a generator matrix of $\C^\perp$. Let $(\hv_i)_{1\leqslant i \leqslant n}$ be the rows of $\Hv$. For all $1\leqslant i \leqslant n, \Supp(\hv_i) = F \implies \C^\perp$ contains $q^n$ codewords of the same support, so the complexity of the algorithm is divided by $q^n$. Thus, the complexity of the attack is
%\[
%\OO{n^3m^3q^{d\Ceiling{\frac{m}{2}} - m - n}}
%\]
%
%There exists a specific attack on the ideal LRPC codes which can be found in \cite{HT15a}. In this article, the authors present an attack against double circulant LRPC codes but it can be adapted straightforwardly in the case of ideal LRPC codes. However, the crucial point of this attack is that the polynomial $X^n-1$ has always $X-1$ as divisor and may have many more factors depending on $n$ and $q$. In the case of ideal LRPC codes, we can choose an irreducible polynomial $P$ of degree $n$ of $\Fq[X]$ to generate the quotient-ring $\Fq[X]/(P)$, which completely negates this specific attack.
%
%
%\subsubsection*{Algebraic attacks}
%\label{subsubsec:AlgebraicAttacks}
%The second way to solve the equations of the system (\ref{eqn:RSD_Fq}) is to use the Groebner basis \cite{LP06}.
%The advantage of these attacks is that they are independent of the size of $q$. They mainly depend on the number of unknowns with respect to the number of equations. However, in the case $q=2$ the number of unknowns is generally too high for that the algorithms by Groebner basis are more efficient than the combinatorial attacks. We have chosen our parameters such that the best attacks are combinatorial, the expected complexity of the algorithms by Groebner basis is based on the article \cite{BFP09}.

\subsection{Best known attacks on $\RSD$}

\label{best_attacks}

The complexity of practical attacks grows very fast with the size of parameters,
there is a structural reason for this: for Hamming distance a key notion
for the attacks consists of counting the number of words of length $n$ and support size $t$,
which corresponds to the Newton binomial coefficient $\binom{n}{t}$, 
whose value is exponential and upper bounded
by $2^n$. In the rank metric case, counting the number of possible supports of size
$r$ for a rank code of length $n$ over $\Fqm$ corresponds to counting the number
of subspaces of dimension $r$ in $\Fqm$: {\bf the Gaussian binomial coefficient}
of size roughly $q^{rm}$, whose value is also exponential but with a quadratic term
in the exponent.

There exist two types of generic attacks on the problem:

- {\bf combinatorial attacks}: these attacks are usually the best ones for small values
of $q$ (typically $q=2$) and when $n$ and $k$ are not too small,
when $q$ increases, the combinatorial aspect makes them less efficient.

The first non-trivial attack on the problem was proposed by Chabaud
and Stern \cite{CS96} in 1996.
It was improved in 2002 by Ourivski and Johannson \cite{OJ02} who proposed
a new attack in $\OO{(n-k)^3m^3q^{(w-1)(k+1)}}$. However, these two attacks did not take account of the value of $m$ in the
exponent. Very recently the two previous attacks were generalized in \cite{GRS16} (and used
to break some repairs of the GPT cryposystems) moreover an algebraic new setting
was also proposed, which gives an attack in $\OO{w^3k^3q^{w\Ceiling{\frac{(w+1)(k+1)-n-1}{w}}}}$. Finally, a last improvement of the combinatorial attack of \cite{GRS16} was proposed this year in \cite{AGHT17}, for a complexity of $\OO{(n-k)^3m^3q^{w\Ceiling{\frac{(k+1)m}{n}}-m}}$.

\begin{remark}
Since the linear system is not random, it is reasonable to take $\omega = 2$ for the choice of the parameters of ROLLO-I, ROLLO-II and ROLLO-III, even if the attack described in \cite{AGHT18} takes $\omega = 3$.

Let us remark that the choice of our parameter is flexible. We could  take $\omega = 0$ and increase the parameters, which corresponds to only keeping the exponential complexity of the attack, for instance by slightly increasing $m$.
\end{remark}


- {\bf algebraic attacks}: the particular nature of the rank metric makes it a natural field
for algebraic attacks and solving by Groebner basis, since these attacks 
are largely independent of the value of $q$
and in some cases may also be largely independent of $m$.
These attacks are usually the most efficient ones when $q$ increases.
There exist different types of algebraic equations settings to try to solve
a multivariate system with Groebner basis.
The algebraic context proposed by Levy and Perret \cite{LP06} in 2006 
considers a quadratic setting over $\Fq$ 
by taking as unknowns the support $E$ of the error and the error
coordinates regarding $E$. It is also possible to consider
the Kernel attack by \cite{FLP08} and the minor approach \cite{FSS10SV} 
which give multivariate equations of degree $r+1$ over $\Fq$ obtained from minors of matrices
Finally,
the recent annulator setting by Gaborit et {\it al.} in \cite{GRS16}
(which is valid on certain type of parameters but may not be independent on $m$)
give multivariate sparse equations of degree $q^{r+1}$ but on the large field
$\Fqm$ rather than on the base field $\Fq$. The latter attack is based on the
notion of $q$-polynomial \cite{O33} and is particularly efficient when $r$ is small.
Moreover, all these attacks can be declined in an hybrid approach where some
unknowns are guessed. In practice (and for the case of this paper)
for the known state of the art these attacks seem less efficient than combinatorial attacks.
Moreover, with today's knowledge, these attacks cannot benefit from a quantum
speed up, hence even if such attacks do a little better for classical security than 256 bits,
it won't necessarily imply a difference for a quantum security of 128 bits.

\subsubsection{Impact of quantum algorithms on the complexity of the attacks}
In post-quantum cryptography, it is important to study the impact of quantum computer on the security of the schemes. In rank metric cryptography, the problems on which we are based are still difficult for a quantum computer, however there is a quantum speedup based on a generalization of Grover’s quantum search algorithm for combinatorial attacks: the exponent of the complexity is divided by 2 \cite{GHT16}, which lead to a complexity of $\OO{(n-k)^3m^3q^{\frac{w}{2}\Ceiling{\frac{(k+1)m}{n}}-m}}$.

Concerning the algebraic attacks, there is currently no quantum speedup as far as we know.




\subsection{Parameters}
\label{subsec:Parameters}

\begin{table*}[bt]\label{table:ParameterKEM}
\centering
\begin{tabular}{|c|c|c|c|}
\hline
Security			&	128				&	192					&	256 \\
\hline
$n$ 				&	47				&	53					&	67\\
\hline
$m$ 				&	71				&	89					&	113\\
\hline
$d$					&	6				&	7					& 	8\\
\hline
$r$					&	5				&	6					&	7\\
\hline
$P$ 				& $X^{47}+X^5+1$	& $X^{53}+X^6+X^2+X+1$	& $X^{67}+X^5+X^2+X+1$\\
\hline
Structural Attack 	&	130				&	207					&	312\\
\hline
Generic Attack 		&	146				&	221					&	329\\
\hline
$p_f$ 				&	$2^{-30}$		&	$2^{-32}$			&	$2^{-36}$\\
\hline
Entropy				&	311				&	499					&	743\\
\hline
Public key (bits)	&	3337			&	4717				&	7571\\
\hline
\end{tabular}
\caption{Examples of parameters of our KEM \ref{subsec:KEM}}
\end{table*}

\begin{table*}[bt]\label{table:ParameterProbaFailure-64}
\centering
\begin{tabular}{|c|c|c|c|}
\hline
Security			&	128				&	192					&	256 \\
\hline
$n$ 				&	83				&	83					&	89\\
\hline
$m$ 				&	71				&	101					&	107\\
\hline
$d$					&	7				&	7					& 	8\\
\hline
$r$					&	5				&	5					&	6\\
\hline
$P$ 				& $X^{83}+X^7+X^4+X^2+1$	& $X^{83}+X^7+X^4+X^2+1$	& $X^{89}+X^{38}+1$\\
\hline
Structural Attack 	&	133				&	209					&	273\\
\hline
Generic Attack 		&	144				&	195					&	260\\
\hline
$p_f$ 				&	$2^{-64}$		&	$2^{-64}$			&	$2^{-64}$\\
\hline
Entropy				&	331				&	481					&	607\\
\hline
Public key Size (bits)	&	5893			&	8383			& 9523\\
\hline
\end{tabular}
\caption{Example of parameters of our PKE \ref{subsec:PKE}, $p_f \leqslant 2^{-64}$}
\end{table*}

\begin{table*}[bt]\label{table:ParameterProbaFailure-80}
\centering
\begin{tabular}{|c|c|c|c|}
\hline
Security			&	128				&	192					&	256 \\
\hline
$n$ 				&	101				&	103					&	103\\
\hline
$m$ 				&	79				&	97					&	107\\
\hline
$d$					&	7				&	8					& 	8\\
\hline
$r$					&	5				&	6					&	6\\
\hline
$P$ 				& $X^{101}+X^7+X^6+X+1$	& $X^{103}+X^9+1$	& $X^{103}+X^9+1$\\
\hline
Structural Attack 	&	136				&	229					&	259\\
\hline
Generic Attack 		&	157				&	234					&	260\\
\hline
$p_f$ 				&	$2^{-80}$		&	$2^{-80}$			&	$2^{-80}$\\
\hline
Entropy				&	371				&	547					&	607\\
\hline
Public key Size (bits)	&	7979		&	9991				& 	11021\\
\hline
\end{tabular}
\caption{Example of parameters of our PKE \ref{subsec:PKE}, $p_f\leqslant 2^{-80}$}
\end{table*}

In this section, we give some sets of parameters for a quantum security parameters level of $64$, $96$ and $128$, corresponding to classical level of security with respect to combinatorial attack of $128$, $192$ and $256$. In all cases, we have chosen $q = 2$. The choice of these parameters depends on the probability of decryption failure and the complexity of the attacks against our cryptosystem:
\begin{enumerate}
\item Message attacks: they consist in solving an instance of the $\IRSR$ problem of weight $r$ \ref{prob:I-RSR}.
\item Attacks on the secret key: they consist to recover the structure of the Ideal-LRPC code by computing a codeword of weight $d$ in the dual code \ref{prob:IndLRPC}.
\item Spurious key attack: as in the NTRU case (see \cite{HPS98})
this attack corresponds to finding small word
vectors in $\Hv$ with rank slightly greater than $d$, and to use
them for decoding. Although theoretically possible, this attack is not doable 
in practice since the fact that $\Hv$ contains small weight vectors implies
that many words of weight $2d$ exist. We do not go into details in this article
but as for MDPC codes \cite{MTSB12}, when the weight increases the complexity of the attacks
grows faster than the number of small weight vectors, so that this attacks - as for NTRU and MDPC- does not work in practice. 
\end{enumerate}
The different parameters are :
\begin{itemize}
\item $n$ is the length the vectors $\hv$ and $\cv$ sent on the public channel.
\item $m$ is the degree of the extension $\Fm$. 
\item $d$ is the weight of the ideal LRPC code used in the protocol.
\item $r$ is the weight of the error.
\item $P$ is the irreducible polynomial of degree $n$ of $\F[X]$ which defines the ideal LRPC code. We have chosen sparse polynomials in order to diminish the computation costs. 
\item the structural attack parameter is the complexity of the best attack to recover the structure of the ideal LRPC code. It consists in looking for a codeword of weight $d$ in an ideal LRPC of type $[2n,n]_{2^m}$ defined by the parity-check matrix $(\Iv_n | \Hv)$ where
\[
\Hv = \begin{pmatrix}
\hv(X) \mod P \\
X\hv(X) \mod P \\
\vdots \\
X^{n-1}\hv(X) \mod P
\end{pmatrix}.
\]

Because of the structure of the ideal LRPC, the complexity of looking for a codeword of weight $d$ is easier than in a random code (see \cite{ABDGHRTZ17a}). The complexity of the attack, for these parameters, is $\OO{(nm)^\omega 2^{d\Ceiling{\frac{m}{2}} - m - n}}$ where $\omega = \log_2 7 \approx 2.8$ is the cost of linear algebra.

\item the generic attack parameter is the complexity of the best attack to recover the support $E$. It consists to solve the I-RSD problem for a random ideal code of type $[2n,n]_{2^m}$ and an error of weight $r$. For our parameters, the complexity of this attack is $\OO{(nm)^\omega 2^{r\Ceiling{\frac{m(n+1)}{2n}} - m}}$ where $\omega = \log_2 7 \approx 2.8$ is the cost of linear algebra.
\item $p_f$ is the probability of failure of the decoding algorithm. We have chosen the parameters such that the theoretic upper bound is below $2^{-26}$ for the KEM. For the PKE, it is necessary to have a lower probability of failure since the public key can be used to encrypt a high number of messages. We give two sets of parameters: the first one for a probability below $2^{-64}$ and the second one for a probability below $2^{-80}$.
\item the entropy parameter is the entropy of the subspace $E$. It is equal to $\log_2 \left( \cg{r}{m} \right)$ and has to be greater than the security parameter. We represent $E$ by a matrix of size $r \times m$ in its row echelon form.
%\item the exchanged data is the number of bits sent by Alice and Bob during the protocol. Since each of them sends one vector of $\Fm^n$, it is equal to $2mn$.
\item the public key size is the number of bits needed to represent the public key $\hv \in \Fqm^n$. It is equal to $mn$.
\end{itemize}

{\bf Comparison with other cryptosystems:} In terms of size of public key,
the system compares very well with other proposal to the NIST competition. 
For 128 bits security key exchange
(in which case one is allowed to a not too small decryption failure rate)
the BIKE proposal (MDPC cryptosystem) has a public key of 10 kilo bits, hence 
the LRPC cryptosystem has public keys roughly three times smaller.
In terms of encryption (with very small or null decryption failure rate), 
the system is comparable to the RQC cryptosystem,
and far smaller than the McEliece cryptosystem.
Globally among all candidates to the NIST competition, the LRPC cryptosystem
has the second smaller size of public keys for 128 bits security, better 
than candidates based on lattices, but a little larger than 
systems based on isogenies. Moreover the system is also efficient in terms
of speed compared to the other NIST proposals.

%\textbf{Quantum speedup:} 

We also provide concrete timings of our implementations (given tables \ref{table:perfmsKEM} and \ref{perfcyclesKEM} for the KEM and tables \ref{perfmsPKE} and \ref{perfcyclesPKE} for the PKE). The benchmarks were performed on an Intel\textregistered Core\texttrademark i7-4700HQ CPU running @ up to 3.40GHz and the software was compiled using GCC (version 6.3.0) with the following command : \texttt{g++ -O2 -pedantic -Wall -Wextra -Wno-vla}.

\begin{table}[h]
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
Security & \KeyGen & \Encap & \Decap\\
\hline
128   &  0.65  & 0.13  & 0.53\\
\hline
192  &  0.73  & 0.13  & 0.88\\
\hline
256 &  0.77  & 0.15  & 1.24\\
\hline
\end{tabular}
\caption{Timings (in ms) of our KEM \ref{subsec:KEM}}
\label{table:perfmsKEM}
\end{center}
\end{table}

\begin{table}[h] 
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
Security & \KeyGen & \Encap & \Decap\\
\hline
128   &  1.58  & 0.30  & 1.27\\
\hline
192  &  1.74  & 0.31  & 2.09\\
\hline
256 &  1.79  & 0.35  & 2.89\\
\hline
\end{tabular}
\caption{Timings (in millions of cycles) of our KEM \ref{subsec:KEM}}
\label{perfcyclesKEM}
\end{center}
\end{table}

\begin{table}[h] 
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
\hline
Security & $p_f$ & \KeyGen & \Encap & \Decap\\
\hline
128 & 64   &  1.09  & 0.22  & 1.04\\
\hline
192 & 64  &  1.33  & 0.23  & 1.08\\
\hline
256 & 64 &  1.51  & 0.25  & 1.58\\
\hline
128 & 80 &  1.51  & 0.29  & 1.16\\
\hline
192 & 80 &  1.82  & 0.36  & 1.80\\
\hline
256 & 80 &  1.94  & 0.31  & 1.68\\
\hline
\end{tabular}
\caption{Timings (in ms) of our PKE \ref{subsec:PKE}}
\label{perfmsPKE}
\end{center}
\end{table}

\begin{table}[h] 
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
\hline
Security & $p_f$ & \KeyGen & \Encap & \Decap\\
\hline
128 & 64   &  2.71  & 0.55  & 2.57\\
\hline
192 & 64  &  3.19  & 0.54  & 1.08\\
\hline
256 & 64 &  3.58  & 0.60  & 3.77\\
\hline
128 & 80 &  3.72  & 0.71  & 2.86\\
\hline
192 & 80 &  4.36  & 0.86  & 4.32\\
\hline
256 & 80 &  4.68  & 0.75  & 4.06\\
\hline
\end{tabular}
\caption{Timings (in millions of cycles) of our PKE \ref{subsec:PKE}}
\label{perfcyclesPKE}
\end{center}
\end{table}
\newpage


==> proof_impact_m.tex <==
\section{Proof of proposition \ref{prop:impact_m}} \label{app:impact_m}

We recall the proposition\ref{prop:impact_m}:

\begin{prop}
Let $E$ be a subspace of $\Fqm$ of dimension $r$. Let $F_1$ and $F_2$ be two subspaces of $\Fqm$ such that \begin{itemize}
\item $\dim F_i = d_i$
\item $\dim (E \cap F_i) = r -c_i$
\end{itemize}
Then $\dim (F_1 \cap  F_2) \geqslant r-c_1-c_2$ and we have
{\small
\[
\prob{(F_1\cap F_2) \subset E} \geqslant \frac{\cg{d_2-r+c_2}{m-d_1-c_1}}{\cg{d_2-r+c_2}{m-r}}q^{(d_1-r+c_1)(d_2-r+c_2)}.
\]
}
If $m \geqslant d_1+d_2$, we have $\prob{(F_1\cap F_2) \subset E} \geqslant 1-\frac{q^{-m+r}(q^{d_1-r+c_1}-1)(q^{d_2-r+c_2}-1)}{q-1} + \OO{q^{-2m}}$ when $m \rightarrow \infty$.
\end{prop}

\begin{proof}
We have:
\begin{IEEEeqnarray}{Rl}
& \dim (F_1 \cap F_2) \geqslant \dim (E \cap F_1 \cap F_2) \nonumber\\
= & \dim (E \cap F_1) + \dim (E \cap F_2) \\&\hspace{2.4cm}- \dim \big( (E \cap F_1) + (E \cap F_2) \big) \nonumber \\
=&2r-c_1-c_2-\dim (E \cap F_1 + E \cap F_2) \nonumber \\
\geqslant &  2r-c_1-c_2-\dim E = r-c_1-c_2. \nonumber
\end{IEEEeqnarray}

For the second point, we need to define the projection over the quotient vector space $\Fqm/E$.
\begin{IEEEeqnarray}{LCCCC}
\text{Let }\varphi & : & \Fqm & \rightarrow & \Fqm/E \nonumber \\
&& \xv & \mapsto & \xv + E \nonumber
\end{IEEEeqnarray}
$\varphi$ is a linear map of $\Fq$ vector spaces. For all $U
\subset \Fqm, U \subset E \iff \varphi(U) = \{0\}$. Moreover we
have the equality $\dim \varphi(U) = \dim U -\dim (E\cap U)$. Therefore,
\[ \left\lbrace \begin{array}{l}
\dim \varphi(F_i) = d_i -r +c_i \nonumber \\
F_1 \cap F_2 \subset E \iff \varphi(F_1 \cap F_2) = \{0\} \nonumber
\end{array}\right. .
\]
Since $\varphi(F_1 \cap F_2) \subset \varphi(F_1)\cap \varphi(F_2)$, $\varphi(F_1)\cap \varphi(F_2) = \{0\} \implies \varphi(F_1 \cap F_2) = \{0\}$. So
\[
\Prob(F_1\cap F_2 \subset E) \geqslant \Prob(\dim (\varphi(F_1)\cap \varphi(F_2)) = 0).
\]
The probability that two subspaces of dimension $a$ and $b$ of a
vector space of dimension $n$ have a null intersection is given by the
formula
$$\frac{\cg{a}{n-b}q^{ab}}{\cg{a}{n}}$$
(see \cite{H14} Proposition 3.2). By taking $n=m-r, a = d_2-r+c_2$ and $b=d_1-r+c_1$, we obtain
{\small
\[
\prob{(F_1\cap F_2) \subset E} \geqslant \frac{\cg{d_2-r+c_2}{m-d_1-c_1}}{\cg{d_2-r+c_2}{m-r}}q^{(d_1-r+c_1)(d_2-r+c_2)}.
\]
}
To compute an approximation, let us use the formula $\cg{a}{n} = \prod_{i=0}^{a-1} \frac{q^n-q^i}{q^a-q^i}$. \label{DvptLimiteProba}
\begin{IEEEeqnarray}{rCCCl}
P_{a,b}(n) &=& \frac{\cg{a}{n-b}q^{ab}}{\cg{a}{n}} & = &  \frac{\displaystyle{\prod_{j=0}^{a-1} \frac{q^{n-b}-q^j}{q^a-q^j}}}{\displaystyle{\prod_{i=0}^{a-1} \frac{q^n-q^i}{q^a-q^i}}}\ q^{ab}\nonumber \\ 
& = & \left(\prod_{i=0}^{a-1} \frac{q^{n-b}-q^i}{q^n-q^i}\right)q^{ab} & = & \prod_{i=0}^{a-1} \frac{q^n-q^{i+b}}{q^n-q^i}  \nonumber \\
 & = & \prod_{i=0}^{a-1} \frac{1-q^{i+b-n}}{1-q^{i-n}}. \nonumber
\end{IEEEeqnarray}
Therefore,
\[
 \ln P_{a,b}(n) = \sum_{i=0}^{a-1} \ln (1-q^{i+b-n}) - \ln (1-q^{i-n}).
\]
$\ln(1-x) = -x+\OO{x^2}$ when $x\rightarrow 0$ hence
\begin{IEEEeqnarray}{rCl}
\ln P_{a,b}(n) & = & \sum_{i=0}^{a-1} \left(q^{i-n} - q^{i+b-n}\right) + \OO{q^{-2n}} \nonumber \\
 &= & q^{-n}(1-q^b) \sum_{i=0}^{a-1} q^i +  \OO{q^{-2n}} \nonumber \\
 & =& -q^{-n}(1-q^b)\frac{q^a-1}{q-1} + \OO{q^{-2n}} \nonumber
\end{IEEEeqnarray}
when $n\rightarrow +\infty$.\\
$e^x = 1+x+\OO{x^2}$ when $x \rightarrow 0 \implies P_{a,b}(n) = 1-\frac{q^{-n}(q^a-1)(q^b-1)}{q-1}+\OO{q^{-2n}}$
By replacing the variables, we obtain
{\small
\begin{IEEEeqnarray}{rcl}
\Prob(F_1\cap F_2 \subset E) \geqslant 1&-&\frac{q^{-m+r}(q^{d_1-r+c_1}-1)(q^{d_2-r+c_2}-1)}{q-1}\nonumber\\
                                        &+& \OO{q^{-2m}}.\nonumber
\end{IEEEeqnarray}
}

\end{proof}

==> syndrome_space_ext_algo.tex <==
\section{Improved decoding : syndrome space expansion algorithm} \label{sec:syndrome space expansion algorithm}

In general, the basic decoding algorithm presented in Section \ref{sec:basicAlgo} does not work when the syndrome space $S = \langle s_1, ..., s_{n-k} \rangle$ is different from $\EF$. In this section, we present an algorithm that can be used between steps 1) and 2) of the basic decoding algorithm to recover $\EF$ in certain cases when $\dim S < \dim \EF$. We denote by $c$ the codimension of $S$ in $\EF$, that is to say $c = \dim \EF - \dim S$.

In this section, we will always suppose that $\dim \EF = rd$ for two reasons:
\begin{itemize}
\item first, according to Proposition \ref{prop:DimensionProductSubspace}, the probability $p_1$ that $\dim \EF < rd$ can easily be exponentially low by increasing $m$. We can also decrease the probability $p_2$ that $S \ne \EF$ by increasing $n$, however for cryptographic applications of LRPC, the parameters of the code are such that $p_1$ is negligible with respect to $p_2$.
\item secondly, the case $\dim \EF = rd$ is the worst case for the decoding since the probability that $S = \EF$ increases when the dimension of $\EF$ decreases. Thus, we can analyze the theoretical probability of failure in the worst case scenario. All the tests we have made show that in practice the probability of failure is smaller when $\dim S < rd$, which confirms our analysis.
\end{itemize}

\subsection{General idea}

This algorithm's aim is to recover vectors of the product space $\EF$ which
do not belong to the syndrome space $S$ by using the structure of the product
space $\EF = \langle f_1e_1, f_2e_1, ..., f_de_r \rangle$ and the fact
that we know a basis $\langle f_1, ..., f_d \rangle$ of $F$. 
%We call a function that increases the dimension of $S$ an ``expansion function''.
We use a function which take on input the subspace $S$ and outputs a subspace $S'$ such that $S \varsubsetneq S' \subset \EF$ with a very high probability, depending on the parameters of the code. We call such a function an ``expansion function''.

Here are two examples of expansion functions:

\begin{enumerate}
\item $f_{decode}(S) =  (S + f_iS_j) \cap (S + f_kS_l)$ is used to decode errors of larger weight.
  %allow increase error weights
\item $f_{prob}(S) = S + FS_{ij} $, where $S_{ij} = S_i \cap S_j$, is used to reduce the decoding failure rate.
\end{enumerate}

We use these expansion functions to describe an iterative algorithm [\ref{fig:Syndrome space expansion algorithm}]. Detailed algorithms for each function are given in the next subsections.

\begin{figure*}[bt]
\centering
\fbox{
  \begin{minipage}{12cm}
  
  {\bf Data:} The syndrome space $S$ and the vector space $F$
  
  {\bf Result:} The expanded syndrome space $S'$, which may be $\EF$, or failure
\begin{enumerate}
\item {\bf Expand $S$ with the expansion function}

Use the expansion function for all possible parameters:\\
$S \leftarrow f_{expand}(S)$

\medskip

\item {\bf Iterative step}

If $\dim S = rd$, then return $S$. If $\dim S < rd$, go back to step~1. If $\dim S$ does not increase during step 1, return failure.

 \end{enumerate}
  \end{minipage}
} \caption{The syndrome space expansion algorithm}
\label{fig:Syndrome space expansion algorithm}
\end{figure*}

\begin{prop} \label{prop:dimSi}
$\dim (S_i \cap E) \geqslant r-c$, with $c = \dim \EF - \dim S$.
\end{prop}

\begin{proof}
We have $\dim S_i = \dim S = rd -c$ and
\begin{IEEEeqnarray}{rCl}
\dim (E+S_i) & = & \dim f_i(E+S_i) = \dim (f_i E+S) \nonumber \\
&\leqslant &\dim \EF =rd
\end{IEEEeqnarray}
since $f_i E$ and $S$ are subspaces of $\EF$.
Hence:
\begin{IEEEeqnarray}{rCCCCCl}
\dim (S_i \cap E)	&	 = 		& \dim E	& +	& \dim S_i	& -	& \dim (E +S_i)\nonumber \\
				& \geqslant	& r			& +	& rd-c		& -	& rd \nonumber \\
				& \geqslant	& r-c. \nonumber
\end{IEEEeqnarray} 
\end{proof}

As we will see in the next subsections, each expansion function has
advantages and drawbacks, and the choice of which function to use
depends on the parameters. In particular, $m$ needs to be high enough
for these functions to work. The function $f_{decode}$ needs $m \ge 3rd-2$ and allows to decode
errors of weight up to $\frac{2}{3}(n-k)$ whereas the function $f_{prob}$ only needs $m \ge 2rd-r$. In this case
we can only decode errors of weight up to $\frac{(n-k)}{2}$ but by strongly reducing the decoding failure probability. In particular, this latter case corresponds to parameters used for cryptography, where $rd \approx (n-k)=\frac{n}{2}$ and $m \approx n$.

\subsection{Increasing the weight of the decoded error vectors}

In this subsection we explain in details the function $f_{decode}$ (the algorithm is described figure \ref{fig:expansion1}).
\[
f_{decode} : S \mapsto (S + f_iS_j) \cap (S + f_kS_l).
\]
The idea is
that each subspace of the form $(S + f_iS_j)$ has a chance to contain
vectors $x$ such that $x \in \EF$ and $x \notin S$, since $\EF \cap f_iS_j \ne \{0\}$. If we find some new vectors of $\EF$ but not the whole product space, we can
reuse values of $(i, j, k, l)$ already tested because they may lead us
to recover some new vectors thanks to the one we have added. Hence the algorithm functions in an iterative way. If during a whole iteration, the dimension of $S$ does not increase, then the algorithm will fail.

\begin{figure}
\begin{algorithmic}[1]
\State \textbf{Input:} The syndrome space $S$ and the vector space $F$
\State \textbf{Output:} The expanded syndrome space $S'$, which may be $\EF$, or failure
	\While{\textit{true}}
		\State $tmp \leftarrow \dim S$ \;
		\For{Every $(i, j, k, l)$ such that $i \neq j$, $k \neq l$ and $(i, j) \neq (k, l)$}
			\State $S \leftarrow (S + f_i.S_j) \cap (S + f_k.S_l)$ \;
		\EndFor
		\If{$\dim S = rd$}
			\Return{$S$} \;
		\EndIf
		\If{$\dim S = tmp$}
			\Return{failure} \;
		\EndIf
	\EndWhile
\end{algorithmic}
\caption{Syndrome space expansion using $f_{decode}$}
\label{fig:expansion1}
\end{figure}

\paragraph{Maximum weight of the decoded errors.}

Without using the syndrome space expansion algorithm, the decoding
algorithm for LRPC codes can decode up to $r = \frac{n-k}{d}$
errors. We can use $f_{decode}$ to deal with error vectors of increased weight.

\begin{theorem}
For $d=2$, under the assumption that $\dim (S_i \cap E) = r-c$ for $1 \leqslant i \leqslant 2$, $f_{decode}$ allows to decode errors of weight up to $r \leqslant \Floor{\frac{2}{3}(n-k)}$ with probability $\approx 1 - \frac{q^{3r-2(n-k)}}{q-1}$ for the general case and errors of weight up to  $r=\frac{2}{3}(n-k)$ with probability $\approx 0.29$ for the case $q=2$.
\end{theorem}

\proof
%In the case $d=2$, when computing $\EF + f_i.f_j^{-1}.\EF$, the expected dimension of this vector space is $rd + r(d-1) = 3r$, since $r$ vectors of $f_i.f_j^{-1}.\EF$ will already be in $\EF$ and the other ones are random. If we get smaller vector spaces when computing $S + f_i.f_j^{-1}.S$ then it means that we can not find the whole space $\EF$, which leads to a decoding failure.
%
%Since the dimension of $S$ is at most $n-k$, the dimension of $S + f_i.f_j^{-1}.S$ is at most $2(n-k)$, which leads to the following inequality : $3r \leqslant 2(n-k)$, hence the result.
%
%In the $d=2$ case, the only expansion that can be done is $S \leftarrow (S + f_1.f_2^{-1}.S) \cap (S + f_2.f_1^{-1}.S)$, hence there is no iterative effect. As $(S + f_1.f_2^{-1}.S) = f_1f_2^{-1}(S + f_2.f_1^{-1}.S)$, the dimension of the two terms is the same. Considering $S$ and $f_1.f_2^{-1}.S$ are independent, the probability of failure is the probability that two subspaces of $\EF + f_i.f_j^{-1}.\EF$ of dimension $n-k$ do not generate the whole space, which is roughly $0.28$ for $q=2$ and close to $q^{-1}$ for $q>2$.
$d=2 \implies \dim \EF = 2r$.\\
Thus, the dimension of $\EF+ f_1f_2^{-1}\EF$ is at most $3r$ for $f_1 E \subset \EF \cap f_1f_2^{-1}\EF$. The only expansion that can be done is $S \leftarrow (S + f_1f_2^{-1}S) \cap (S + f_2f_1^{-1}S)$, hence there is no iterative effect.

 Since $(S + f_1f_2^{-1}S) = f_1f_2^{-1}(S + f_2f_1^{-1}S)$, the dimension of these two vectors spaces is the same. If  $ \dim (S + f_1 f_2^{-1}S) < 3r$, then it is impossible to find the whole space $\EF$, which leads to a decoding failure. Since the dimension of $S$ is at most $n-k$, the dimension of $S + f_if_j^{-1}S$ is at most $2(n-k)$, which implies $3r \leqslant 2(n-k)$. Hence $r \leqslant \Floor{\frac{2}{3}(n-k)}$.
 
 Considering that $S$ and $f_1f_2^{-1}S$ are independent, the probability of success is the probability that the sum of two subspaces of dimension $n-k$ of $\EF + f_1f_2^{-1}\EF$ generates the whole space. So we have:
\begin{IEEEeqnarray}{rCl}
p_{success} & =& \Prob (S + f_1 f_2^{-1}S = \EF + f_1f_2^{-1}\EF)  \nonumber \\
& = & \Prob (\dim (S + f_1 f_2^{-1}S) = 3r) \nonumber \\
& =& \Prob (2(n-k) - \dim S \cap (f_1 f_2^{-1}S) = 3r) \nonumber \\
& =& \Prob (\dim S \cap (f_1 f_2^{-1}S) = 2(n-k) - 3r). \nonumber
\end{IEEEeqnarray}
The formula for computing this probability can be found in \cite{H14} (Proposition 3.2). We obtain:
\begin{IEEEeqnarray}{rCl}
p_{success} & =& \frac{\cg{2(n-k)-3r}{n-k}q^{(3r-(n-k))^2}}{\cg{n-k}{3r}} \nonumber \\
 & =& \frac{\cg{3r-(n-k)}{n-k}q^{(3r-(n-k))^2}}{\cg{3r-(n-k)}{3r}}. \label{eqn:ExactFormulaProbSucces|d=2}
\end{IEEEeqnarray}
By applying the series expansion for $P_{a,b}(n)$  (Appendix \ref{app:impact_m},page \pageref{DvptLimiteProba}) with $n=3r, a=b=3r-(n-k)$, we obtain:
\begin{IEEEeqnarray}{rCl}
p_{success} & \approx & 1-\frac{q^{-3r}(q^{3r-(n-k)}-1)^2}{q-1}  \nonumber \\
 & \approx & 1- \frac{q^{3r-2(n-k)}}{q-1}. \nonumber
\end{IEEEeqnarray}

In the case $q=2$ and $3r=2(n-k)$, this approximation is incorrect. According to Equation \eqref{eqn:ExactFormulaProbSucces|d=2},
\begin{IEEEeqnarray}{rCl}
p_{success} & = & \frac{\cgdeux{n-k}{n-k} 2^{(n-k)^2}}{\cgdeux{n-k}{3r}} \nonumber \\
& = & \frac{2^{(n-k)^2}}{\cgdeux{n-k}{2(n-k)}} \nonumber \\
%& = & \frac{2^{(n-k)^2}{\prod_{i=0}^{n-k-1} \frac{2^{2(n-k)}-2^i}{2^{n-k}-2^i}}  \nonumber \\
%& = & \prod_{i=0}^{n-k-1} \frac{2^{2(n-k)}-2^{n-k+i}}{2^{n-k}-2^i} \nonumber \\
& \longrightarrow &  0.29 \text{ when } (n-k)\rightarrow \infty \nonumber \\
&&\text{ (the convergence is very fast)}.\nonumber
\end{IEEEeqnarray}
\qed

In figure \ref{simud2}, we present simulation results comparing the observed probability of failure and $q^{-1}$.

\begin{figure}
        \centering
        \includegraphics[scale=0.6]{fig/figure4_simud2.pdf}
        \caption{Results for $d=2$, $n=30$, $k=15$, $r=10$. We can observe the success rate of $\approx 0.29$ for $q=2$.}
        \label{simud2}
\end{figure}

\begin{proposition}
Under the assumption that $\dim (S_i \cap E) = r-c$ for $1 \leqslant i \leqslant d$, $f_{decode}$ allows to decode errors up to $r \leqslant \frac{n-k}{d-1}$ for $d>2$, using the fact that the algorithm functions in an iterative way.
\end{proposition}

\proof
For $d>2$, the algorithm may recover $\EF$ as long as $c<r$ (i.e there are vectors of $E$ in $S_i$) using the iterative effect, so the algorithm does not have to recover the whole product space at a time : if it recovers one new vector then it can be added to $S$ and used with different values of $(i, j, k, l)$ (even those that have already been used) to produce more vectors, hence the only condition for that method to work is $c<r$ in order to have vectors of $E$ in $S_i$.

If the $n-k$ syndrome vectors are independent, then $c$ is $rd - (n-k)$, which gives the result:

\begin{IEEEeqnarray}{rCl}
c < r & \Leftrightarrow & rd-(n-k)<r \nonumber \\
      & \Leftrightarrow & r(d-1)<n-k \nonumber \\
      & \Leftrightarrow & r<\frac{n-k}{d-1}. \nonumber
\end{IEEEeqnarray}
\qed

Although giving a theorical probability of failure is difficult in this case since there is an iterative effect, simulations show that in practice we attain this bound.

\paragraph{Minimal value of $m$}

\begin{proposition}
$f_{decode}$ recovers new vectors of $\EF$ only if $m > 3rd - 2$
\end{proposition}

\proof
To produce vectors of $\EF$, we compute vector spaces of the form $f_if_j^{-1}S$. If we suppose that $f_j^{-1}S$ contains exactly $r-c$ independent vectors of $E$, which is the worst case, then we get $r-c$ vectors of $\EF$ and $r(d-1) + c$ random vectors in $S'_{ij} = f_if_j^{-1}S$. 

By adding this vector space to $S$, the dimension cannot exceed $rd + r(d-1) + c = 2rd - r + c$ i.e the dimension of $\EF$ along with the random vectors in $S'_{ij}$.

The intersection between $S'_{ij}$ and $S'_{kl}$ needs to remove all the random vectors in order to recover vectors that are $\in \EF$, whence:

\begin{IEEEeqnarray}{rl}
                  & \dim(S'_{ij}) + \dim(S'_{kl}) \leqslant m + \dim(S'_{ij} \cap S'_{kl}) \nonumber\\
\Leftrightarrow & 2(2rd - r + c) \leqslant m + rd \nonumber \\
\Leftrightarrow & m \geqslant 4rd - 2r + 2c - rd \nonumber \\
\Leftrightarrow & m \geqslant 3rd - 2r + 2c. \nonumber
\end{IEEEeqnarray}

Since $c$ can not be higher than $r-1$ (there would be no vectors of $E$ in $f_j^{-1}S$), the inequality becomes $m \geqslant 3rd - 2$.
\qed

The value of $m$ needed by this expansion function is pretty high and does not fit the parameters used for cryptography. However, it works for $d=2$, which is not the case of $f_{prob}$ studied in the next subsection.

\subsection{Reducing the decryption failure rate}

\subsubsection{Description of the algorithm}

In this subsection we will study $f_{prob}$ in a more detailed
way (the algorithm is described figure \ref{fig:expansion2}. 
\[
f_{prob} : S \mapsto S + FS_{ij}.
\]
This function fits the parameters used for cryptography and is
used to reduce the decoding failure rate. It uses the fact that
$S_{ij} = S_i \cap S_j$ contains at least $r-2c$ independent vectors of $E$ (see Proposition \ref{prop:dim Sij cap E}) and is a subspace of $E$ with a very high probability when $m$ is large enough. Thus, the subspace $FS_{ij}$ has a chance to contain a vector $x \in \EF$ and $x \notin S$.\\
\begin{figure}[h]
\begin{algorithmic}[1]
\State \textbf{Input:} The syndrome space $S$ and the vector space $F$
\State \textbf{Output:} The expanded syndrome space $S'$, which may be $\EF$, or failure

	\While{\textit{true}}
		\State $tmp \leftarrow \dim S$ \;
		\For{Every $(i, j)$ such that $i \neq j$}
			\State $S \leftarrow S + FS_{ij}$ \;
		\EndFor
		\If{$\dim S = rd$}
			\Return{$S$} \;
		\EndIf
		\If{$\dim S = tmp$}
			\Return{failure} \;
		\EndIf
	\EndWhile
\end{algorithmic}
\caption{Syndrome space expansion using $f_{prob}$}
\label{fig:expansion2}
\end{figure}

\begin{proposition}\label{prop:dim Sij cap E}
$\dim (S_{ij} \cap E) \geqslant r-2c$ for all $i,j \in [1..d]$, with $c = \dim \EF - \dim S$.
\end{proposition}

\proof
Using Proposition \ref{prop:dimSi}, a simple computation gives us the result:
\begin{IEEEeqnarray}{rCl}
\dim (S_{ij}\cap E)	&=& \dim (S_i\cap S_j \cap E)  \nonumber \\
					&=&  \dim (S_i \cap E) + \dim (S_j \cap E)	\nonumber \\
					& &- \dim \big( (S_i \cap E)+(S_j \cap E)\big) \nonumber \\
					&\geqslant & 2(r-c) 					- r \nonumber \\
					&\geqslant & r-2c. \nonumber
\end{IEEEeqnarray}
\qed

\begin{theorem}
Let $\Prob(c=l)$ be the probability that $\dim \EF - \dim S = l$ and
let $\Prob_{c=l}(failure)$ be the probability that the syndrome space expansion algorithm does not recover $\EF$ when $c=l$.
Using the syndrome space expansion algorithm with $f_{prob}$, the probability of failure is :

$$\prob{c \geqslant \frac{r}{2}} + \sum\limits_{l=1}^{\Floor{\frac{r}{2}} - 1} \Prob(c=l) \times \Prob_{c=l}(failure).$$

\end{theorem}

\proof
The main source of decoding failures for the basic decoding algorithm is the fact that the syndrome coordinates do not generate the whole product space $\EF$, so we need to compute the global probability of not recovering $\EF$ using $f_{prob}$.

When $c \geqslant \frac{r}{2}$, in general $S_{ij}$ is empty so the syndrome space expansion algorithm will not recover $\EF$, which leads to a failure.

When $c < \frac{r}{2}$, the probability that the syndrome space expansion algorithm recovers $\EF$ is $\Prob_{c=l}(failure)$. We multiply this probability by the probability of $c$ being equal to $l$ to get the overall probability of not recovering $\EF$.
\qed

\begin{proposition} \label{prop:prob_c_eq_l}
$\Prob(c=l) \simeq q^{-l(n-k-rd+l)}$
\end{proposition}

\proof

The probability that the $n-k$ syndrome coordinates generate a subspace of codimension $l$ of $\EF$ is the probability that a random $(n-k) \times rd$ matrix in $\Fq$ is of rank $rd - l$. From \cite{L06}, we have that $S_t$, the number of $m \times n$ matrix of rank $t$, is :

$$S_t = \prod_{j=0}^{t-1} \frac{(q^n - q^j)(q^m - q^j)}{(q^t - q^j)}.$$

We can approximate this formula by ignoring $q^j$, which leads to :

$$S_t \simeq \prod_{j=0}^{t-1} \frac{(q^n)(q^m)}{(q^t)} = \prod_{j=0}^{t-1} q^{n + m - t} = q^{t(n+m-t)}.$$

From that, we deduce the number of $(n-k) \times rd$ matrices of rank $rd - l$ :

$$q^{(rd-l)(n-k+rd-rd+l)} = q^{(rd-l)(n-k+l)}.$$

By dividing this quantity by the total number of $(n-k) \times rd$ matrices, we get the probability that a random matrix has rank $rd -l$ :

\begin{IEEEeqnarray}{rCl}
\frac{q^{(rd-l)(n-k+l)}}{q^{(n-k)rd}} &=& q^{(rd-l)(n-k+l) - (n-k)rd}\nonumber \\
                                      &=& q^{lrd - l(n-k) - l^2}\nonumber \\
                                      &=& q^{-l(n-k-rd+l)}\nonumber
\end{IEEEeqnarray}

Hence the result. \qed

\subsubsection{Case of codimension 1}

Before giving the probability of success of Algorithm \ref{fig:expansion2}, we need the following lemma:

\begin{lemma} \label{dimSicapE}
The dimension of $S_i \cap E$ is :
\begin{itemize}
\item $r$ with probability $p_r = \frac{\cg{r}{rd-1}}{\cg{r}{rd}} \approx q^{-r}$.
\item $r-1$ with probability $1-p_r \approx 1 - q^{-r}$.
\end{itemize}
\end{lemma}
\begin{proof}
  We have:
$\dim S_i \cap E = r \iff E \subset S_i \iff f_iE \subset S$.\\
The space $f_iE$ is a subspace of dimension $r$ of $\EF$ and $S$ is a random subspace of dimension $rd-1$ of $\EF$, hence
\[
\Prob(\dim (S_i \cap E) = r) = \frac{\cg{r}{rd-1}}{\cg{r}{rd}} \approx q^{-r}
\]
which proves the first point.
According to Proposition \ref{prop:dimSi}, $\dim (S_i \cap E) \geqslant r-1$ which concludes the proof of this lemma.
\end{proof}

We can now give the probability of success of the decoding algorithm in the case $\dim S = \dim \EF -1$.

\begin{theorem} \label{failure_exp2}
Under the assumption $S_{ij} \subset E$ and $\dim S
= \dim \EF -1$, the syndrome space expansion algorithm
using $f_{prob}$ recovers $\EF$ with probability at least
$1-q^{(2-r)(d-2)}$.
\end{theorem}

\proof 

To find an upper bound on the probability of failure, we are going to
focus on the case where $\dim(S_{ij} \cap E) = r-2$. Indeed, Lemma
\ref{dimSicapE} shows that the typical dimension of $S_i \cap E$ is
$r-1$. Furthermore, when there exists $i$ such that $\dim(S_i \cap E)
= r$, the algorithm has access to more vectors of $E$ and so this
leads to a smaller probability of failure. The same thing goes for the
case where there exists $\dim(S_{ij}) = r-1$ instead of $r-2$ which is
the expected size, so we can consider that $\dim(S_{ij}) = r-2$ since
this will lead to an upper bound of the probability of failure.
% Pas très bien dit %%%%%Juste pas lisible !

We are now going to study the dimension of $S_{ij} + S_{jk} + S_{ik}$. There are two possibilities:

\begin{itemize}
\item If $S_{ij} = S_{jk}$, then necessarily we have $S_{ik} = S_{ij} = S_{jk}$, because the $r-2$ vectors of $S_{ij} + S_{jk}$ are both in $S_i$ and $S_k$. This happens with probability $q^{2-r}$ : the probability that two subspaces of dimension $r-2$ ($S_{ij}$ and $S_{jk}$) of a vector space of dimension $r-1$ ($S_j \cap E$) are equal.
\item If $S_{ij} \neq S_{jk}$, then we have $S_{ik} + S_{ij} + S_{jk} = E$ : we know that $S_{ik} + S_{ij} = S_{i} \cap E$, and that $S_{jk} \not\subset S_i$ (otherwise we would be in the first case). Hence $S_{ik} + S_{ij} + S_{jk} = E$.
\end{itemize}

If there exists a set $\{S_{i_1j_1}, \dots, S_{i_nj_n}\}$ such that their direct sum equals $E$, then the algorithm will succeed since it will have added exactly $\EF$ to $S$ at one point. If such a set does not exist, then it means that every $S_{ij}$ are equal to each other. In particular, every vector of $E$ the algorithm as access to is $\in S_1, \dots, \in S_d$, which means that when we multiply this vector by $F$, the resulting vectors will already be in $S$ and we will obtain no information, causing the algorithm to fail.

The probability that all the $S_{ij}$ are equal is the probability of $S_{12} = S_{23} = \dots = S_{d-1,d}$. Since $d-2$ equalities are needed, the probability of this happening is $q^{(2-r)(d-2)}$, which gives the probability of failure. \qed

\paragraph{Impact of $m$ on decoding.}

If the value of $m$ is not high enough, then $S_{ij}$ will contain not only vectors of $E$ but also random vectors. When this happens, the $S_{ij}$ cannot be used by the expansion algorithm because it would add random vectors to $S$.

\begin{prop} \label{prop:impact_m}
Let $E$ be a subspace of $\Fqm$ of dimension $r$. Let $F_1$ and $F_2$ be two subspaces of $\Fqm$ such that \begin{itemize}
\item $\dim F_i = d_i$
\item $\dim (E \cap F_i) = r -c_i$
\end{itemize}
Then $\dim (F_1 \cap  F_2) \geqslant r-c_1-c_2$ and we have
{\small
\[
\prob{(F_1\cap F_2) \subset E} \geqslant \frac{\cg{d_2-r+c_2}{m-d_1-c_1}}{\cg{d_2-r+c_2}{m-r}}q^{(d_1-r+c_1)(d_2-r+c_2)}.
\]
}
If $m \geqslant d_1+d_2$, we have $\prob{(F_1\cap F_2) \subset E} \geqslant 1-\frac{q^{-m+r}(q^{d_1-r+c_1}-1)(q^{d_2-r+c_2}-1)}{q-1} + \OO{q^{-2m}}$ when $m \rightarrow \infty$.
\end{prop}

The proof of this proposition is given appendix \ref{app:impact_m}.

\begin{cor} \label{cor:formule_m}
Applying Proposition \ref{prop:impact_m} with $F_i = S_i$, $\dim S_i = rd-1$ and $c_i = 1$, we obtain $\prob{(S_i\cap S_j) \subset E} \approx 1 - \frac{q^{-m+2rd-r}}{q-1}$.
\end{cor}

From corollary \ref{cor:formule_m}, we can see that adding $1$ to the value of $m$ leads to a factor $q^{-1}$ in the probability of finding random vectors in $S_{ij}$, thus this probability can be made arbitrarily small.

To detect that $S_{ij}$ contains random vectors, we can keep track of the dimension of $S$ during the expansion. Indeed, if $S_{ij}$ contains random vectors, adding $FS_{ij}$ to $S$ will lead to a dimension greater than $rd$. In this case we just need to discard the vectors we just added and continue with the next $S_{ij}$.

\paragraph{Comments on the small values of $q$}

When using small values of $q$, the cases where $\dim S_i \cap E$ or
$\dim S_{ij} > r-2$ are not so rare. Simulation for $d=3, r=3$ seems
to show that the probability $q^{(2-r)(d-2)}$ is accurate when $q$ is
high enough, but is a pessimistic bound when $q$ is small, especially
when $q=2$. Simulation results are shown in figure \ref{fig:simud3r3}. 

\begin{figure}
\centering
\includegraphics[scale=0.6]{fig/figure6_simud3r3.pdf}
\caption{Simulation results for $c=1$, $d=3, r=3$}
\label{fig:simud3r3}
\end{figure}

\begin{proposition}
For $q=2$, the syndrome space expansion algorithm using $f_{prob}$ recovers $\EF$ with probability at least $1-q^{(1-r)(d-2)}$.
\end{proposition}

\proof When $q=2$, the probability that $S_{ij} = S_{jk}$ used in the proof above is not $q^{2-r}$ but $q^{1-r}$. Indeed, from Proposition \ref{prop:impact_m}, we get that the probability of $S_{ij}$ and $S_{jk}$ being equal is approximately $\frac{q^{-1}}{q-1}$ which is equal to $q^{-1}$ when $q=2$. \qed

This leads to a failure probability of $q^{(1-r)(d-2)}$. This is still not as good as what happens in practice, since it does not take into account the fact that the algorithm often has more than $r-2$ vectors of $E$ in each $S_{ij}$ to work with, but is a closer estimate in this special case.

\subsubsection{Case of codimension $\geqslant$ 2}

In the case $c \geqslant 2$, we have no theoretical analysis, but we can do simulations for particular parameters to estimate the probability of failure. In practice we obtain good estimations of the probability of failure. For example, for $q=2$, $c=2$, $r=5$, $d=6$ and $m=80$, we obtain a probability of failure of $2^{-14}$.

\subsubsection{Upper bound on the decryption failure rate}

\begin{itemize}
\item The codimension of $S$ in $\EF$ is 1, but the algorithm fails to recover $\EF$.
\item The codimension of $S$ in $\EF$ is greater than 1. Since it is difficult to give a theorical bound on the probability, we will consider that decoding fails in that case:
\end{itemize}

%To summarize : the probability of the codimension of $S$ in $\EF$ being 1 is $q^{(n-k)-rd}$ (proposition \label{prop:failure prob}), and the algorithm fails with probability $q^{(2-r)(d-2)}$ (theorem \ref{failure_exp2}) when this is the case. The algorithm can also fail because of the codimension being greater than 1, which happens with probability $\simeq q^{-2(n-k-rd+2)}$ (proposition \ref{prop:prob_c_eq_l}), and we consider that the algorithm fails in that case. That gives us the following upper bound of the decryption failure rate :

$$q^{(2-r)(d-2)} \times q^{(n-k)-rd} + q^{-2(n-k-rd+2)}.$$

\subsection{Tradeoff between expansion functions}

In the previous subsections we studied two expansion functions in detail:

\begin{itemize}
\item $f_{decode}$ can decode higher values of $r$ but needs a higher $m$ ($m \ge 3rd-r$) 
\item $f_{prob}$ fits values of $m$ ($m \ge 2rd-r$) used in cryptography, but is less effective since it decodes up to $c < \frac{r}{2}$ instead of $c < r$
\end{itemize}

Depending on the parameters, we can build new expansion functions: in general, the higher $m$ is, the better the expansion function will be. For example, if $m$ is really high, we can use this function: $S \leftarrow (S + f_iS_j + f_kS_l) \cap (S + f_aS_b + f_cS_d)$ which is basically an improvement of $f_{decode}$ since it has a higher chance of recovering vectors of $EF$ by adding two $f_iS_j$ at a time.

If $m$ is lower than the one needed for $f_{prob}$, one can use the function $S \leftarrow S + F(S_{ij} \cap S_k)$ which requires a lower $m$ but can only decode with $c < \frac{r}{3}$.

\subsection{Rank Support Recovery algorithm}

Algorithm \ref{fig:Decoding algorithm of LRPC codes} computes the error vector from the syndrome equations $\Hv\ev^T=\sv^T$. However, for cryptographic applications, we may just recover the support of the error and use it as the shared secret since the $I-RSR$ and $I-RSD$ problems are equivalent. We use the Rank Support Recovery (RSR) algorithm \ref{algo:RSR} which is a shortened version of the decoding algorithm \ref{fig:Decoding algorithm of LRPC codes} which does not compute the coordinates of the error, and uses $f_{prob}$ to reduce the decoding failure rate.

\begin{figure}
\begin{algorithmic}[1]
\State \textbf{Input:} A parity-check matrix $\Hv \in \Fqm^{(n-k)\times n}$ of support $F$ of dimension $d$ of an LRPC code, a syndrome $\sv \in \Fqm^{n-k}$, an integer $r$.
\State \textbf{Output:} A subspace $E$ of dimension $\leqslant r$ such that it exists $\ev \in \Fqm^n$ of support $E$ with $\Hv\ev^T=\sv^T$.

\State Compute the syndrome space $S=\vect{s_1,\cdots,s_{n-k}}$ \;
\State Use the syndrome space expansion algorithm described in Algorithm \ref{fig:expansion2} \;
\State Define $S_i=f_i^{-1}\EF$ then compute the support of the error $E = S_1 \cap S_2 \cap \cdots \cap S_d$\;
\Return $E$

\end{algorithmic}
\caption{the Rank Support Recovery algorithm}
\label{algo:RSR}
\end{figure}

Algorithm \ref{fig:expansion2} allows to reduce the decryption
failure rate by a factor $q^{(2-r)(d-2)}$. However, this algorithm
takes a variable number of iterations to terminate, which may lead to
big  variations in the global execution time. In particular, if one
can determine whether the syndrome space expansion algorithm was
needed or not, the execution time may leak some information. To
prevent that, we present a variation of the syndrome space recovery
algorithm [\ref{algo:crypto_expansion}] that performs a fixed number of intersections and still fits the proof of Theorem~\ref{failure_exp2}.

\begin{figure}
\begin{algorithmic}[1]
\State \textbf{Input:} The syndrome space $S$ and the vector space $F$
\State \textbf{Output:} The expanded syndrome space $S'$, which may be $\EF$

\For{$i$ from 1 to $d-1$}
	\State Precompute $S_{i, i+1}$ \;
\EndFor
\For{$i$ from 1 to $d-2$}
	\State $tmp \leftarrow S + F(S_{i, i+1} \oplus S_{i+1, i+2} \oplus S_{i, i+2})$ \;
	\If{$\dim tmp \leqslant rd$}
		\State $S \leftarrow tmp$ \;
		%\State \tcc{$tmp$ is used to check that $m$ has no impact, has in proposition \ref{prop:impact_m}}
	\EndIf
\EndFor
\Return{$S$}
\end{algorithmic}
\caption{Syndrome space expansion algorithm used in cryptography}
\label{algo:crypto_expansion}
\end{figure}

\subsection{Complexity of the decoding algorithm}

Algorithms \ref{fig:expansion1} and \ref{fig:expansion2} are iterative algorithms, hence their exact complexity is hard to study precisely. We can however give an upper bound of their complexity, by noticing that the maximum number of iterations before the algorithms finishes is at most $c$: indeed, $c$ must decrease at each iteration, otherwise the algorithms will stop returning $failure$.

\begin{proposition} \label{prop:comp_fdecode}
The number of operations in $\Fq$ for the syndrome space expansion algorithm using $f_{decode}$ in algorithm \ref{fig:expansion1} is bounded above by:

$$ c \times d(d-1)\times(d(d-1)-1) \times 16 r^2 d^2 m$$
\end{proposition}

\begin{proof}
As said before, the complexity of this algorithm can be bounded by $c$ times the cost of an iteration. When using $f_{decode}$, the most costly operation is the computation of the intersection. Intersecting two vector spaces of dimension $2rd$ costs $16 r^2 d^2 m$ operations in $\Fq$, and $d(d-1)\times(d(d-1)-1)$ different values are possible for $(i, j, k, l)$ at each iteration, hence the result.
\end{proof}


\begin{proposition} \label{prop:comp_fprob}
The number of operations in $\Fq$ for the syndrome space expansion algorithm using $f_{prob}$ in algorithm \ref{fig:expansion2} is bounded above by :

$$ c \times d(d-1) \times 4 r^2 d^2 m$$
\end{proposition}

\begin{proof}
The proof is the same as for proposition \ref{prop:comp_fdecode}, except that the most costly step of each iteration is the computation of the $S_{ij}$. Intersecting two vector spaces of dimension $rd$ costs $4 r^2 d^2 m$ operations in $\Fq$, and there are $d(d-1)$ $S_{ij}$ to compute at each iteration, hence the result.
\end{proof}

In order to allow constant time implementations, the syndrome space expansion algorithm used in the cryptographic context computes a fixed number of intersections, so its complexity can be derived easily:

\begin{proposition}
The number of operations in $\Fq$ for the syndrome space expansion algorithm used
in the cryptographic context in algorithm \ref{algo:crypto_expansion} is:

$$ ((d-1)+(d-2)) \times 4r^2d^2m$$
\end{proposition}

\begin{proof}
As for Proposition~\ref{prop:comp_fprob}, the most costly step of this algorithm is the computation of every $S_{ij}$. Each intersection costs $4 r^2 d^2 m$, and the structure of the algorithm allows to reduce the number of intersections to $(d-1)+(d-2)$, hence the result.
\end{proof}

In practice the algorithm for cryptographic applications is very efficient, and
for the iterative case, the upper bound is scarcely met since the algorithm
usually stops before doing the maximum number of possible iterations.


